Using Deep Learning to Find the Next Unicorn: A Practical Synthesis

Startups often represent newly established business models associated with disruptive innovation and high scalability. They are commonly regarded as powerful engines for economic and social development. Meanwhile, startups are heavily constrained by many factors such as limited financial funding and human resources. Therefore, the chance for a startup to eventually succeed is as rare as "spotting a unicorn in the wild". Venture Capital (VC) strives to identify and invest in unicorn startups during their early stages, hoping to gain a high return. To avoid entirely relying on human domain expertise and intuition, investors usually employ data-driven approaches to forecast the success probability of startups. Over the past two decades, the industry has gone through a paradigm shift moving from conventional statistical approaches towards becoming machine-learning (ML) based. Notably, the rapid growth of data volume and variety is quickly ushering in deep learning (DL), a subset of ML, as a potentially superior approach in terms of capacity and expressivity. In this work, we carry out a literature review and synthesis on DL-based approaches, covering the entire DL life cycle. The objective is a) to obtain a thorough and in-depth understanding of the methodologies for startup evaluation using DL, and b) to distil valuable and actionable learning for practitioners. To the best of our knowledge, our work is the first of this kind.

==> sections/title_authors.tex <==
%--------------------------------------------------------%
%	TITLE SECTION with authors
%--------------------------------------------------------%

% Article title
  \title{\vspace{-15mm}\fontsize{21pt}{10pt}\selectfont\textbf{Wordy Manuscript Title: \\Even Wordier Manuscript Subtitle\thanks{Draft manuscript. Please do not cite without the authors' permission.}}}

% Authors and Affiliations
  \author[1]{\large First Author}
  \author[1]{\large Second Author}
  \author[2]{\large Third Author}
  \affil[1]{\normalsize Department of XYZ, The University of ABC}
  \affil[2]{\normalsize Department of ABC, The University of XYZ}
  \renewcommand\Authands{ and }

% Today's date
	\date{Submitted: \usvardate\today}

==> sections/title_noauthors.tex <==
%-----------------------------------------------------------
%	TITLE SECTION - with authors
%-----------------------------------------------------------

% Article title
  \title{\vspace{-15mm}\fontsize{21pt}{10pt}\selectfont\textbf{Use Deep Learning to Find the Next Unicorn: A Practical Synthesis\thanks{Anonymous draft manuscript. Please do not share or cite without the authors' permission.}}}

% Today's date
	\date{Submitted: \usvardate\today}

\makeatletter
\renewcommand{\@maketitle}{
\newpage
 \null
 \vskip 2em%
 \begin{center}%
  {\LARGE \@title \par}%
 \end{center}%
 \par} \makeatother

